Building Squares with Optimal State Complexity in Restricted Active Self-Assembly

Tile Automata is a recently defined model of self-assembly that borrows many concepts from cellular automata to create active self-assembling systems where changes may be occurring within an assembly without requiring attachment. This model has been shown to be powerful, but many fundamental questions have yet to be explored. Here, we study the state complexity of assembling $n \times n$ squares in seeded Tile Automata systems where growth starts from a seed and tiles may attach one at a time, similar to the abstract Tile Assembly Model. We provide optimal bounds for three classes of seeded Tile Automata systems (all without detachment), which vary in the amount of complexity allowed in the transition rules. We show that, in general, seeded Tile Automata systems require $\Theta{(\log^{\frac{1}{4}} n)}$ states. For single-transition systems, where only one state may change in a transition rule, we show a bound of $\Theta{(\log^{\frac{1}{3}} n)}$, and for deterministic systems, where each pair of states may only have one associated transition rule, a bound of $\Theta( (\frac{\log n}{\log \log n})^\frac{1}{2} )$.

==> lowerStringsAlt.tex <==
\subsection{Strings}
In this section we formulate the concept of self-assembling a binary string, and provide lower bounds for doing so.  In this formulation, we map a potentially large $n\times m$ block subassembly to either $0$ or $1$, 



Here we provide lower bounds on building binary strings.These bounds hold at any scale. We define scaled strings using macroblocks. A macroblock is an $a \times b$ subassembly which maps to a specific bit of the string. Let $M^{a,b}(\Sigma)$ be the set of all size $a \times b$ macroblocks over states $\Sigma$. Let the $i$th macroblock of an assembly be the size $a \times b$ subassembly whose lower left tile is at location $(ai, 0)$.

\begin{definition}[String Representation]
An assembly $A$ over states $\Sigma$ represent a string $S$ over a set of symbols $U$ at scale $a \times b$ if there exists a mapping from the elements of $M^{a,b}(\Sigma)$ to the elements of $U$, and the $i$th macroblock of $A'$ maps to the $i$th symbol of $S$.
\end{definition}

% \begin{definition}[String Representation]
%An assembly $A$ over states $\Sigma$ represent a string $S$ over a set of symbols $U$ at scale $a \times b$ if there exists a mapping from the elements of $\Sigma$ to the elements of $U$ and subassembly $A'  \sqsubset A$, such that for each state at location $(x, y)$ represents the $i$th bit of $S$ for $ia \leq x < i(a+1)$, $0 \leq y < b$.
%\end{definition}

\begin{lemma}
Let $U$ be a set of TA systems and $b$ be a one-to-one function mapping each element of $U$ to a string of bits, and $S$ be a Kolmogorov Random string, then any TA system $\Gamma \in U$  that uniquely assembles an assembly $A$ that represents $S$ at any scale has $|b(\Gamma)| \geq |S|$.
\end{lemma}
\begin{proof}
Given the string $b(\Gamma)$ the assembly $A$ can be computed and the string $S$ be output after reading from each macroblock.
Since $S$ is Kolmogorov Random the shortest program which outputs $S$ is of length $|S|$ so
$b(\Gamma) \geq |S|$.
\end{proof}

\begin{theorem}[Deterministic TA]
For all $n > 0$, there exists a binary string $S$ of length $n$, such that any deterministic Tile Automata that uniquely assembles an assembly that represents $S$ at any scale contains $\Omega(n^\frac{1}{2})$ states.
\end{theorem}


\begin{theorem}[Single-Transition TA]
For all $n > 0$, there exists a binary string $S$ of length $n$, such that any single-transition Tile Automata that uniquely assembles an assembly that represents $S$ at any scale contains $\Omega(n^\frac{1}{3})$ states.
\end{theorem}

\begin{theorem}[Nondeterministic TA]
For all $n > 0$, there exists a binary string $S$ of length $n$, such that any Tile Automata (in particular any nondeterministic system) that uniquely assembles an assembly that represents $S$ at any scale contains $\Omega(n^\frac{1}{4})$ states.
\end{theorem} 

==> sCRN.tex <==
\section{Comparison to Surface Chemical Reaction Networks}
Key differences between sCRNs and seeded Tile Automata are as follows,

\begin{itemize}
	\item Surface CRNs are usually defined starting on a finite subset of the grid with each vertex/tile having a starting state, while Tile Automata starts from a subset of the 
\end{itemize} 
 
 
 - Formulate Problem
